Collective Phenomena in Defect Crystals

We investigate effects of interactions between substitutional defects on the properties of defect crystals at low temperatures, where defect motion is governed by quantum effects. Both, thermal and dynamical properties are considered. The influence of interactions on defect motion is described via a collective effect. Our treatment is semiclassical in the sense that we analyze collective effects in a classical setting, and analyze the influence on quantized defect motion only thereafter. Our theory describes a crossover to glassy behavior at sufficiently high defect concentration. Our approach is meant to be general. For the sake of definiteness, we evaluate most of our results with parameters appropriate for Li-doped KCl crystals.

==> entete.tex <==
\input epsf.tex
\textheight 245mm
\setcounter{page}{1}
\pagestyle{plain}
\makeatletter
\def\refrule{%
\end{multicols}\widetext\vglue13pt %
\hskip10.25pc\rule{20pc}{.1mm}\hfill %
\vglue.14cm\begin{multicols}{2}\narrowtext %
}

\def\references{%
\list{\@biblabel{\arabic{enumiv}}}%
{\labelwidth\WidestRefLabelThusFar  \labelsep2pt %
\leftmargin\labelwidth %
\advance\leftmargin\labelsep %
\ifdim\baselinestretch pt>1 pt %
\parsep  4pt\relax %
\else   %
\parsep  0pt\relax %
\fi
\itemsep\parsep %
\usecounter{enumiv}%
\let\p@enumiv\@empty
\def\theenumiv{\arabic{enumiv}}%
}%
\let\newblock\relax %
\sloppy\clubpenalty4000\widowpenalty4000
\sfcode`\.=1000\relax
\ifpreprintsty\else\small\fi
}

% Headings, different for even/odd and first.
% Enter TITLE and AUTHORS by hand (!! shift first head if first page even !!)

  \def\AUTHORS{\rmtop  REIMER K\"UHN AND ALOIS W\"URGER}
  \def\JOURNAL{PHYSICAL REVIEW B}
  \def\DATE{SUBMITTED}%
  \def\TITLE{\rmtop COLLECTIVE PHENOMENA IN DEFECT CRYSTALS}
  \def\VOLUME{}
  \def\NUMBER{}
  \def\PAGE{1}

\newfont{\rmtop}{cmr10 at 9pt}

  \def\ps@plain{%
  \gdef\@oddhead{\ifnum\thepage=\PAGE {\hbox to 2in{\rmtop\JOURNAL%
  \hfil}\hfil{{\rmtop VOLUME \VOLUME, NUMBER \NUMBER}}\hfil\hbox to %
  2in{\hfil{\rmtop\DATE}}}\else{\hbox to %
  1in{$\underline{\hbox{\rmtop\VOLUME}}$\hfil}\hfil\TITLE\hfil\hbox to %
  1in{\hfil\rmtop\thepage}}\fi}%
  \gdef\@evenhead{\ifnum\thepage=\PAGE {\hbox to 2in{\rmtop\JOURNAL%
  \hfil}\hfil{{\rmtop VOLUME \VOLUME, NUMBER \NUMBER}}\hfil\hbox to %
  2in{\hfil{\rmtop\DATE}}}\else{\hbox to %
  1in{\rmtop\thepage\hfil}\hfil\AUTHORS%
  \hfil\hbox to 1in{\hfil$\underline{\hbox{\rmtop\VOLUME}}$}}\fi}%
  \gdef\@oddfoot{\ifnum\thepage=\PAGE{\hbox to %
  2.5in{\hfil}\hfil$\ \ \underline{\hbox{\rmtop\VOLUME}}\ \ \ \ \ \ %
  ${\rmtop\thepage}%
  \hfil\hbox to 2.5in{\hfil Typeset using REV\TeX}}\else{}\fi}%
  \gdef\@evenfoot{\ifnum\thepage=\PAGE{\hbox to %
  2.5in{\hfil}\hfil$\ \ \underline{\hbox{\rmtop\VOLUME}}\ \ \ \ \ \ %
  ${\rmtop\thepage}%
  \hfil\hbox to 2.5in{\hfil Typeset using REV\TeX}}\else{}\fi}%
  }%


  \makeatother

